On Capacity of the Writing onto Fast Fading Dirt Channel

The "Writing onto Fast Fading Dirt" (WFFD) channel is investigated to study the effects of partial channel knowledge on the capacity of the "writing on dirty paper" channel. The WFFD channel is the Gel'fand-Pinsker channel in which the output is obtained as the sum of the input, white Gaussian noise and a fading-times-state term. The fading-times-state term is equal to the element-wise product of the channel state sequence, known only at the transmitter, and a fast fading process, known only at the receiver. We consider the case of Gaussian distributed channel states and derive an approximate characterization of capacity for different classes of fading distributions, both continuous and discrete. In particular, we prove that if the fading distribution concentrates in a sufficiently small interval, then capacity is approximately equal to the AWGN capacity times the probability of this interval. We also show that there exists a class of fading distributions for which having the transmitter treat the fading-times-state term as additional noise closely approaches capacity. Although a closed-form expression of the capacity of the general WFFD channel remains unknown, our results show that the presence of fading can severely reduce the usefulness of channel state knowledge at the transmitter.

==> AppPartA.tex <==
\section{ Proof of Lem. \ref{lem:Mean and variance of the fading-time-state term}}
\label{app:Mean and variance of the fading-time-state term}
%
Consider the more general model in \eqref{eq:Dirty Paper Channel}  for which the fading-times-state term is obtained as $\ct {{\At}}^N \circ {{S'}}^N$ with $\At\sim P_A$ and $\St \sim \Ncal(\mu_{\St},\sgs_{\St})$ and $\ct \in \Rbb$, i.e.
\ea{
{\Yt}^N= {X}^N+ \ct {\At}^N \circ  {\St}^N +Z^N.
\label{eq:generalized}
}
%
For the expression in \eqref{eq:generalized}, we notice that
\ea{
%&
%\ct
\At_i \St_i=
%& \quad
 %\ct \lb
 (\St_i-\mu_{\St})(\At_i-\mu_{\At})+\St_i \mu_{\At}+\At_i \mu_{\St} - \mu_{\At} \mu_{\St},
 %\rb.
 % \nonumber
 \label{eq: generalize decompose}
}
and
\ea{
\ct \At_i \St_i = \ct \sigma_{\At} \sigma_{\St} \cdot  \f {\At_i}{ \sigma_{\At} } \cdot \f {\St_i}{ \sigma_{\St} }.
\label{eq:adjust to one}
}
From \eqref{eq: generalize decompose}, we conclude that $\mu_{\At} \mu_{\St}$ and  $\mu_{\St} \At^N$ can be subtracted from the channel output  since the receiver has knowledge of the fading sequence.
%
From this, it follows that  the assumption of $\mu_{\St}=0$ in \eqref{eq:Dirty Paper Channel} is without loss of generality.
%
From \eqref{eq:adjust to one}, we notice that the coefficient $c$ in \eqref{eq:Dirty Paper Channel} can be used to normalize the variance of both fading and state to be unitary.
%
%From \eqref{eq:adjust to one} we can observe that one cannot distinguish
%
Finally, under the assumption that $\mu_{\St}=0$, we can fix $\ct>0$ since the state distribution is symmetric an thus
$c S^N \sim c (-S^N)$.
% 

==> AppPartE.tex <==
\section{Proof of Th. \ref{th:fat-tailed distribution}}
\label{app:fat-tailed distribution}
%
Let us rewrite the distribution in \eqref{eq:fat tail} for $I=[\al_{\min},\al_{\max}]$  with  $\al_{\min}  = \ka c^{-M}$, $ \al_{\max} = \ka$  and some $M \in \Nbb$, as
\ea{
P_A(a)=\f 1 {\log (\al_{\max}/\al_{\min})} \cdot \f 1 a \cdot 1_{\{\al_{\min}\leq a \leq \al_{\min}\}}.
% 1_{\{k c^{-M}\leq a \leq k\}}
\label{eq:dist A 2}
}
%For the distribution in \eqref{eq:dist A 2} we have
with
\ea{
%\mu_A  & = \f {\al_{\max}-\al_{\min}} {\log (\al_{\max}/\al_{\min})} \\
%\sgs_A & = \f 1 2 \f {(\al_{\max}-\al_{\min})(\al_{\max}+\al_{\min}-2)}{\log (\al_{\max}/\al_{\min})}.
\ka= \f {2 M \log(c) c^M}{\sqrt{2 M \log(c)(c^{2M}-1)-4 (c^M-1)^2}},
\label{eq:ka}
}
%
to guarantee unitary variance.
%
In the following, we show that there exists a choice of $M$ as a function of $c$ such that the result in
Th. \ref{th:fat-tailed distribution} holds.
%

%\newpage
%
%%and show that, for such choice, the result in
%
%%
%
%
%%
%%%
%% note that $\ka$ is an increasing function of  $M$ which increases as $\log(M)$ asymptotically.
%%%


In the achievability  proof, we  consider the point-to-point achievable strategy in which $c A^N \circ S^N$ is treated as additional noise, which attains
\ea{
R^{\rm IN} \geq \f 12 \log \lb 1 + \f{P}{1+c(1+\mu_A)} \rb \geq \f 12 \log \lb 1 + \f{P}{1+c} \rb.
\label{eq:inner last}
}
%

\noindent
$\bullet$ {\bf Converse.}
%
%For the converse proof, the derivation is  we consider the model with integer fading-times-state gain  $c'=\lfloor c \rfloor$: according to Lem. \ref{lem:capacity decreasing c} reducing $c$ increases capacity.
%
%
%\newpage
%
We begin by developing the proof for the case of $c$ integer and successively generalized the result to the case of any $c$.
%
For $c$ integer and for the fading distribution in \eqref{eq:dist A 2},  define the random variable $A_{\De}$ to be a quantization of the $A$ obtained in two steps: course quantization followed by fine quantization.
%
In the course quantization, $A$ is quantized in intervals  $I_k=\{[\ka/c^k,\ka/c^{k-1}), \quad k \in[0 \ldots M-1]\}$ while, in the fine quantization, each interval $I_k$ is further subdivided into $c^{M-k}$ intervals of equal probability.
%
Since
%
\ea{
\Pr[k\leq a\leq j] = \Pr[c k\leq a\leq cj],  \quad k,j\in I, k\leq j,
\label{eq:scaling probability}
}%
we have that
\ea{
%P_I & =
 \Pr [\ka/c^k \leq A_{\De} < \ka/c^{k-1}]=\f 1 M   \quad \forall \ k \ \in [0 \ldots  M-1],
}
while
\ea{
\Pr [A_{\De}= j,  \ j\in [\ka/c^k,\ka/c^{k-1}) ]= \f 1 M \f {1}{c^{k-1}(c-1)}.
\label{eq:values j}
}
The values $j$ in \eqref{eq:values j} are chosen as $\Ebb[A | A \in [\ka/c^k,\ka/c^{k-1})]$ so that $\Ebb[A]=\Ebb[A_{\De}]$.
%
Let us represent the  random variable $A_{\De}$   as in the three in Fig. \ref{fig:supp A de}: the $k^{\rm th}$ level in the tree represents the  rough quantization interval $I_k$. The elements on the level represent the $j^{\rm th}$ elements in the fine quantization.
%
The root of the of the trees has $c-1$ outgoing edges, while all the remaining non-leaf nodes have $c$ outgoing edges, so the $k^{\rm th}$  level in the tree has $(c-1)c^{k-1}$ elements.
%
Let also the node $i$ at level $k$ to be connected with the nodes $[ci, \ldots, c(i+1)-1]$ in the $(k+1)^{\rm th}$ level.
%
%\newpage
%
%
%The random variable $A_{\De}$  is schematically represented by the tree in Fig. \ref{fig:supp A de}: the node $i$ in the tree represents the element $\ka/i$.  The tree as $M$ levels and the sum of the probability of the elements on the $k^{\rm th}$ level is $1/M$ while the probability of each note is $1/M \cdot 1/(c-1)^{k}$ where $k$ is the level of the node.

\begin{figure}
  \centering
\begin{tikzpicture}[->,>=stealth',level/.style={sibling distance = 4.75cm/#1,
  level distance = 1.5cm}]
\node [arn_n] {$\cdot$}
  child{ node [arn_n] {1}
            child{ node [arn_n] {$c$}
            	child{ node [arn_n] {$c^2$} edge from parent node[above left]
                         {}} %for a named pointer
                child{  node [arn_n] {\tiny $\ldots$}}
							child{ node [arn_n] {$c^2+c-1$}}
                            %child{ node [arn_n] {$...$}}
            }
            child{  node [arn_n] {\tiny $\ldots$}}
            child{ node [arn_n] {$2c-1$}
							child{ node [arn_n] {$2c^2-c$}}
                            child{  node [arn_n] {\tiny $\ldots$}}
							child{ node [arn_n] {$2c^2-1$}}
            }
    }
   child{  node [arn_n] {\tiny $\ldots$}}
   child{ node [arn_n] {$c-1$}
            child{ node [arn_n] {$c^2-c$}
							child{ node [arn_n] {$c^3-c^2$}}
                            child{  node [arn_n] {\tiny $\ldots$}}
							child{ node [arn_n] {$(c^2-1)(c-1)$}}
            }
  child{  node [arn_n] {\tiny $\ldots$}}
            child{ node [arn_n]{$c^2-1$}
							child{ node [arn_n] {$c^3-c$}}
                              child{  node [arn_n] {\tiny $\ldots$}}
							child{ node [arn_n] {$c^3-1$}}
            }
		}
;
\end{tikzpicture}
  \caption{Representation of the support of $A^{\rm \De}$}
\label{fig:supp A de}
\end{figure}
%

Next, define $\Acal_m$ for $m \in [c^{M-1} \ldots c^{M}-1]$ as the path from the root  of the tree (excluded) to each of the leaves and let $\At_m$ be the random variable uniformly distributed over the set $\Acal_m$.
%
Because of the  property in \eqref{eq:scaling probability}, we conclude that the elements in each set are exponentially spaced apart of a factor $c$.
%
Using the definition of $\At_m$, the random variable $A_{\De}$  can be rewritten as
\ea{
A_{\De}=K \At^T,
\label{eq: basis}
}
where $K$ is uniformly distributed over the set of natural basis of
 $\Rbb^{c^{M-1}(c-1)}$, i.e. all the sequences of length $c^{M-1}(c-1)$  of the form $[0\ldots 0,1, 0 \ldots 0]$, while $\At=[\At_{c^{M-1}} \ldots \At_{c^M-1}]$.
%
The equality in \eqref{eq: basis} holds because each element at the $k^{\rm th}$ level appears $c^{M-1-k}(c-1)$ times in the set $\At$,
while the probability of selecting a particular $\At_j$ is $1/(c^{M-1}(c-1))$.


The next step in the proof is to apply the result in Th. \ref{thm:approximate capacity strong} to each random variable $\At_{j}$,
since the elements in the support $\Acal_m$ satisfy the strong fading conditions.
%
To this end, note that the derivation in \eqref{eq:fano} can be adapted as
\ean{
 N(R- \ep_N)  &
 \leq I(Y^N;W|A^N) \\
 & =   H(Y^N|A^N)-H(Y^N|W,A^N) \\
%
& = H(Y^N|A^N)-\sum_{K^N} P_{K^N}(k^N) H(Y^N|W,A^N,k^N).
%
%& \leq H(Y^N|A^N)-\sum_{k^N \in \Tcal(P_K)} P_{K^N}(k^N) H(Y^N|W,\At^N,k^N).
}
%Since $K$ is uniformly distributed, each element of $\At$ appears in the same fraction: accordingly
%
For each term $H(Y^N|W,A^N,k^N)$, we can repeat the argument in the proof  Th. \ref{thm:approximate capacity strong} and construct $M-1$ ``complementary sequences'' in the spirit of \eqref{eq:definition ao}.
% in which the elements in $\At_j$ are permuted in each sequence..
%
Note that, in general, the condition in \eqref{eq:strong fading intro 1} does not hold for $\At_k$ so that this bounding yields
\ean{
 H(Y^N|W,\at^N,k^N)
& \leq \f 1  M  \sum_{\at^N} \lb H(Y^N|W,\at^N,k^N)+ H(Y^N|W,\at^N_{(2)},k^N)\ldots  H(Y^N|W,\at^N_{(M)},k^N) \rb \\
%
& \leq \f {M-2} {M} \log(c^2)+1.
}
By choosing $M$ sufficiently large, we have  $1/{M} \log(c^2) \leq 1$ so the approach in  Th. \ref{thm:approximate capacity strong} yields the outer bound
\ea{
R^{\rm OUT} = \f 12 \log \lb 1 + \f {P}{c^2(1+\mu_{A_{\De}})+1}\rb +G_s+1,
}
for $G_s$ in \eqref{eq:outer bound gap strong}.
%
%\newpage
%
The term $G_s$ is small for $\mu_A$ small: the mean of $A$ is obtained as
\ea{
\mu_A  & = \f {\al_{\max}-\al_{\min}} {\log (\al_{\max}/\al_{\min})},
}
and $\mu_{A_{\De}} = \mu_A$ so that, for $M$ large, $\mu_A<1$ and, consequently, $G_s \leq 1$.
%
%

The final step is to apply arguments similar to Th. \ref{th:narrow fading} to conclude that, for $M$ sufficiently large,  the distance in the elements of the support of $A_{\De}$ is smaller than $1/c$ so that the capacity of the channel with fading distribution $A$ is to within $1 \ \bpcu$ from the capacity of the channel with fading distribution $A_{\De}$.
%
The overall gap between the inner bound in \eqref{eq:inner last} and the outer bound is then obtained as $G_s+1+1/2 \leq 5/2$.

\medskip

The above derivation holds for $c$ integer: for a general $c$ repeat the above derivation for $c'=\lfloor c \rfloor$ since, according to Lem. \ref{lem:capacity decreasing c} reducing $c$ increases capacity.
%
On the other hand, since $\lfloor c \rfloor<2c$, capacity of the channel with parameter $c'$ is of at most half a bit larger than the capacity of the channel with parameter $c$: this further adds $1/2 \ \bpcu$ to the gap  between the inner bound
and so that the total gap for $c \in \Rbb$ is at most $3 \ \bpcu$.
%


